Forecasting Workload in Cloud Computing: Towards Uncertainty-Aware Predictions and Transfer Learning

Predicting future resource demand in Cloud Computing is essential for optimizing the trade-off between serving customers' requests efficiently and minimizing the provisioning cost. Modelling prediction uncertainty is also desirable to better inform the resource decision-making process, but research in this field is under-investigated. In this paper, we propose univariate and bivariate Bayesian deep learning models that provide predictions of future workload demand and its uncertainty. We run extensive experiments on Google and Alibaba clusters, where we first train our models with datasets from different cloud providers and compare them with LSTM-based baselines. Results show that modelling the uncertainty of predictions has a positive impact on performance, especially on service level metrics, because uncertainty quantification can be tailored to desired target service levels that are critical in cloud applications. Moreover, we investigate whether our models benefit transfer learning capabilities across different domains, i.e. dataset distributions. Experiments on the same workload datasets reveal that acceptable transfer learning performance can be achieved within the same provider (because distributions are more similar). Also, domain knowledge does not transfer when the source and target domains are very different (e.g. from different providers), but this performance degradation can be mitigated by increasing the training set size of the source domain.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> references.tex <==
@article{kim2020forecasting,
  title={Forecasting cloud application workloads with cloudinsight for predictive resource management},
  author={Kim, In Kee and Wang, Wei and Qi, Yanjun and Humphrey, Marty},
  journal={IEEE Transactions on Cloud Computing},
  year={2020},
  publisher={IEEE}
}

@inproceedings{khan2012workload,
  title={Workload characterization and prediction in the cloud: A multiple time series approach},
  author={Khan, Arijit and Yan, Xifeng and Tao, Shu and Anerousis, Nikos},
  booktitle={2012 IEEE Network Operations and Management Symposium},
  pages={1287--1294},
  year={2012},
  organization={IEEE}
}

@article{diebold2002comparing,
  title={Comparing predictive accuracy},
  author={Diebold, Francis X and Mariano, Robert S},
  journal={Journal of Business \& economic statistics},
  volume={20},
  number={1},
  pages={134--144},
  year={2002},
  publisher={Taylor \& Francis}
}

@article{breusch1979simple,
  title={A simple test for heteroscedasticity and random coefficient variation},
  author={Breusch, Trevor S and Pagan, Adrian R},
  journal={Econometrica: Journal of the econometric society},
  pages={1287--1294},
  year={1979},
  publisher={JSTOR}
}

@article{koot2021usage,
  title={Usage impact on data center electricity needs: A system dynamic forecasting model},
  author={Koot, Martijn and Wijnhoven, Fons},
  journal={Applied Energy},
  volume={291},
  pages={116798},
  year={2021},
  publisher={Elsevier}
}

@article{du2003univariate,
  title={Univariate versus multivariate time series forecasting: an application to international tourism demand},
  author={Du Preez, Johann and Witt, Stephen F},
  journal={International Journal of Forecasting},
  volume={19},
  number={3},
  pages={435--451},
  year={2003},
  publisher={Elsevier}
}

@article{chayama2016univariate,
  title={When univariate model-free time series prediction is better than multivariate},
  author={Chayama, Masayoshi and Hirata, Yoshito},
  journal={Physics Letters A},
  volume={380},
  number={31-32},
  pages={2359--2365},
  year={2016},
  publisher={Elsevier}
}

@article{belkhir2018assessing,
  title={Assessing ICT global emissions footprint: Trends to 2040 \& recommendations},
  author={Belkhir, Lotfi and Elmeligi, Ahmed},
  journal={Journal of cleaner production},
  volume={177},
  pages={448--463},
  year={2018},
  publisher={Elsevier}
}

@article{calheiros2014workload,
  title={Workload prediction using ARIMA model and its impact on cloud applications’ QoS},
  author={Calheiros, Rodrigo N and Masoumi, Enayat and Ranjan, Rajiv and Buyya, Rajkumar},
  journal={IEEE transactions on cloud computing},
  volume={3},
  number={4},
  pages={449--458},
  year={2014},
  publisher={IEEE}
}

@article{ruan2022cloud,
  title={Cloud Workload Turning Points Prediction via Cloud Feature-Enhanced Deep Learning},
  author={Ruan, Li and Bai, Yu and Li, Shaoning and Lv, Jiaxun and Zhang, Tianyuan and Xiao, Limin and Fang, Haiguang and Wang, Chunhao and Xue, Yunzhi},
  journal={IEEE Transactions on Cloud Computing},
  year={2022},
  publisher={IEEE}
}

@article{baldan2016forecasting,
  title={A forecasting methodology for workload forecasting in cloud systems},
  author={Baldan, Francisco J and Ramirez-Gallego, Sergio and Bergmeir, Christoph and Herrera, Francisco and Benitez, Jose M},
  journal={IEEE Transactions on Cloud Computing},
  volume={6},
  number={4},
  pages={929--941},
  year={2016},
  publisher={IEEE}
}

@inproceedings{rossi2022bayesian,
  title={Bayesian uncertainty modelling for cloud workload prediction},
  author={Rossi, Andrea and Visentin, Andrea and Prestwich, Steven and Brown, Kenneth N},
  booktitle={2022 IEEE 15th International Conference on Cloud Computing (CLOUD)},
  pages={19--29},
  year={2022},
  organization={IEEE}
}

@inproceedings{leka2021hybrid,
  title={A Hybrid CNN-LSTM Model for Virtual Machine Workload Forecasting in Cloud Data Center},
  author={Leka, Habte Lejebo and Fengli, Zhang and Kenea, Ayantu Tesfaye and Tegene, Abebe Tamrat and Atandoh, Peter and Hundera, Negalign Wake},
  booktitle={2021 18th International Computer Conference on Wavelet Active Media Technology and Information Processing (ICCWAMTIP)},
  pages={474--478},
  year={2021},
  organization={IEEE}
}

@inproceedings{pushpalatha2021amalgamation,
  title={Amalgamation of Neural Network and Genetic Algorithm for Efficient Workload Prediction in Data Center},
  author={Pushpalatha, R and Ramesh, B},
  booktitle={Advances in VLSI, Signal Processing, Power Electronics, IoT, Communication and Embedded Systems: Select Proceedings of VSPICE 2020},
  pages={69--84},
  year={2021},
  organization={Springer}
}

@article{talahmeh2021time,
  title={Time Series Prediction of Server Workload Using Hybrid Model of Recurrent Neural Network and Genetic Algorithms},
  author={Talahmeh, Amin and Awad, Mohammed and Eleyat, Mujahed and others},
  year={2021},
  journal={The International Journal of Engineering \& Science},
  volume={10},
  pages={1--10}
}

@inproceedings{dang2021multivariate,
  title={Multivariate Deep Learning Model For Workload Prediction In Cloud Computing},
  author={Dang-Quang, Nhat-Minh and Yoo, Myungsik},
  booktitle={2021 International Conference on Information and Communication Technology Convergence (ICTC)},
  pages={858--862},
  year={2021},
  organization={IEEE}
}

@article{ouhame2021efficient,
  title={An efficient forecasting approach for resource utilization in cloud data center using CNN-LSTM model},
  author={Ouhame, Soukaina and Hadi, Youssef and Ullah, Arif},
  journal={Neural Computing and Applications},
  pages={1--13},
  year={2021},
  publisher={Springer}
}

@inproceedings{xi2021attention,
  title={An Attention-based Recurrent Neural Network for Resource Usage Prediction in Cloud Data Center},
  author={Xi, Huidan and Yan, Cheng and Li, Huixi and Xiao, Yinhao},
  booktitle={Journal of Physics: Conference Series},
  volume={2006},
  number={1},
  pages={012007},
  year={2021},
  organization={IOP Publishing}
}

@inproceedings{qian2021attention,
  title={An Attention-based GRU Encoder Decoder for Hostload Prediction in a Data Center},
  author={Qian, Shengpan and Yu, Yang and Li, Ling and Chang, Yanbo},
  booktitle={2021 International Conference on Computer Communication and Artificial Intelligence (CCAI)},
  pages={121--125},
  year={2021},
  organization={IEEE}
}

@article{patel2022hybrid,
  title={A hybrid CNN-LSTM model for predicting server load in cloud computing},
  author={Patel, Eva and Kushwaha, Dharmender Singh},
  journal={The Journal of Supercomputing},
  pages={1--30},
  year={2022},
  publisher={Springer}
}

@article{valarmathi2021resource,
  title={Resource utilization prediction technique in cloud using knowledge based ensemble random forest with LSTM model},
  author={Valarmathi, K and Kanaga Suba Raja, S},
  journal={Concurrent Engineering},
  volume={29},
  number={4},
  pages={396--404},
  year={2021},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{zhang2022multi,
  title={A multi-output prediction model for physical machine resource usage in cloud data centers},
  author={Zhang, Yongde and Liu, Fagui and Wang, Bin and Lin, Weiwei and Zhong, Guoxiang and Xu, Minxian and Li, Keqin},
  journal={Future Generation Computer Systems},
  year={2022},
  volume = {130},
  pages = {292-306},
  publisher={Elsevier}
}

@article{zhang2018efficient,
  title={An efficient deep learning model to predict cloud workload for industry informatics},
  author={Zhang, Qingchen and Yang, Laurence T and Yan, Zheng and Chen, Zhikui and Li, Peng},
  journal={IEEE transactions on industrial informatics},
  volume={14},
  number={7},
  pages={3170--3178},
  year={2018},
  publisher={IEEE}
}

@article{yazdanian2021e2lg,
  title={E2LG: a multiscale ensemble of LSTM/GAN deep learning architecture for multistep-ahead cloud workload prediction},
  author={Yazdanian, Peyman and Sharifian, Saeed},
  journal={The Journal of Supercomputing},
  volume={77},
  pages={1--31},
  year={2021},
  publisher={Springer}
}

@article{karim2021bhyprec,
  title={BHyPreC: a novel Bi-LSTM based hybrid recurrent neural network model to predict the CPU workload of cloud virtual machine},
  author={Karim, Md Ebtidaul and Maswood, Mirza Mohd Shahriar and Das, Sunanda and Alharbi, Abdullah G},
  journal={IEEE Access},
  volume={9},
  pages={131476--131495},
  year={2021},
  publisher={IEEE}
}

@article{banerjee2021efficient,
  title={Efficient resource utilization using multi-step-ahead workload prediction technique in cloud},
  author={Banerjee, Sounak and Roy, Sarbani and Khatua, Sunirmal},
  journal={The Journal of Supercomputing},
  volume={77},
  pages={1--28},
  year={2021},
  publisher={Springer}
}

@article{bi2021integrated,
  title={Integrated deep learning method for workload and resource prediction in cloud systems},
  author={Bi, Jing and Li, Shuang and Yuan, Haitao and Zhou, MengChu},
  journal={Neurocomputing},
  volume={424},
  pages={35--48},
  year={2021},
  publisher={Elsevier}
}

@article{kumar2021self,
  title={Self directed learning based workload forecasting model for cloud resource management},
  author={Kumar, Jitendra and Singh, Ashutosh Kumar and Buyya, Rajkumar},
  journal={Information Sciences},
  volume={543},
  pages={345--366},
  year={2021},
  publisher={Elsevier}
}

@article{hao2021transfer,
  title={Transfer learning of Bayesian network for measuring QoS of virtual machines},
  author={Hao, Jia and Yue, Kun and Zhang, Binbin and Duan, Liang and Fu, Xiaodong},
  journal={Applied Intelligence},
  volume={51},
  number={12},
  pages={8641--8660},
  year={2021},
  publisher={Springer}
}

@article{khan2022workload,
  title={Workload forecasting and energy state estimation in cloud data centres: ML-centric approach},
  author={Khan, Tahseen and Tian, Wenhong and Ilager, Shashikant and Buyya, Rajkumar},
  journal={Future Generation Computer Systems},
  volume={128},
  pages={320--332},
  year={2022},
  publisher={Elsevier}
}

@article{salinas2020deepar,
  title={DeepAR: Probabilistic forecasting with autoregressive recurrent networks},
  author={Salinas, David and Flunkert, Valentin and Gasthaus, Jan and Januschowski, Tim},
  journal={International Journal of Forecasting},
  volume={36},
  number={3},
  pages={1181--1191},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{fawaz2018transfer,
  title={Transfer learning for time series classification},
  author={Fawaz, Hassan Ismail and Forestier, Germain and Weber, Jonathan and Idoumghar, Lhassane and Muller, Pierre-Alain},
  booktitle={2018 IEEE international conference on big data (Big Data)},
  pages={1367--1376},
  year={2018},
  organization={IEEE}
}

@article{he2022multivariate,
  title={Multivariate Time Series Deep Spatiotemporal Forecasting with Graph Neural Network},
  author={He, Zichao and Zhao, Chunna and Huang, Yaqun},
  journal={Applied Sciences},
  volume={12},
  number={11},
  pages={5731},
  year={2022},
  publisher={Multidisciplinary Digital Publishing Institute}
}

%%%%%%%%

@article{muller2015benefits,
  title={Benefits of cloud computing: literature review in a maturity model perspective},
  author={M{\"u}ller, Sune Dueholm and Holm, Stefan Rub{\ae}k and S{\o}ndergaard, Jens},
  journal={Communications of the Association for Information Systems},
  volume={37},
  number={1},
  pages={42},
  year={2015}
}

@book{marr2020tech,
  title={Tech Trends in Practice: The 25 Technologies that are Driving the 4th Industrial Revolution},
  author={Marr, Bernard},
  year={2020},
  publisher={John Wiley \& Sons}
}

@article{idg2020idg,
author = {{IDG Communications Inc.}},
institution = {International Data Group},
year = {2020},
title = {{IDG} Cloud Computing Survey 2020}}

@inproceedings{tirmazi2020borg,
  title={Borg: the next generation},
  author={Tirmazi, Muhammad and Barker, Adam and Deng, Nan and Haque, Md E and Qin, Zhijing Gene and Hand, Steven and Harchol-Balter, Mor and Wilkes, John},
  booktitle={Proceedings of the Fifteenth European Conference on Computer Systems},
  pages={1--14},
  year={2020}
}

@article{borghesi2018scheduling,
  title={Scheduling-based power capping in high performance computing systems},
  author={Borghesi, Andrea and Bartolini, Andrea and Lombardi, Michele and Milano, Michela and Benini, Luca},
  journal={Sustainable Computing: Informatics and Systems},
  volume={19},
  pages={1--13},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{jelassi2017survey,
  title={A survey on quality of service in cloud computing},
  author={Jelassi, Mariem and Ghazel, Cherif and Sa{\"\i}dane, Leila Azzouz},
  booktitle={2017 3rd International Conference on Frontiers of Signal Processing (ICFSP)},
  pages={63--67},
  year={2017},
  organization={IEEE}
}

@article{vazquez2015,
author = {Vazquez, C. and Krishnan, R. and John, E.},
journal = {Journal of Wireless Mobile Networks, Ubiquitous Computing, and Dependable Applications},
year = {2015},
pages = {87-110},
title = {Time series forecasting of cloud data center workloads for dynamic resource provisioning},
volume = {6}
}

@inproceedings{di2012host,
  title={Host load prediction in a {Google} compute cloud with a {Bayesian} model},
  author={Di, Sheng and Kondo, Derrick and Cirne, Walfredo},
  booktitle={SC'12: Proceedings of the International Conference on High Performance Computing, Networking, Storage and Analysis},
  pages={1--11},
  year={2012},
  organization={IEEE}
}

@article{hu2014efficient,
  title={Efficient resources provisioning based on load forecasting in cloud},
  author={Hu, Rongdong and Jiang, Jingfei and Liu, Guangming and Wang, Lixin},
  journal={The Scientific World Journal},
  volume={2014},
  year={2014},
  publisher={Hindawi}
}

@inproceedings{gao2020machine,
  title={Machine learning based workload prediction in cloud computing},
  author={Gao, Jiechao and Wang, Haoyu and Shen, Haiying},
  booktitle={2020 29th international conference on computer communications and networks (ICCCN)},
  pages={1--9},
  year={2020},
  organization={IEEE}
}

@article{song2018host,
  title={Host load prediction with long short-term memory in cloud computing},
  author={Song, Binbin and Yu, Yao and Zhou, Yu and Wang, Ziqiang and Du, Sidan},
  journal={The Journal of Supercomputing},
  volume={74},
  number={12},
  pages={6554--6568},
  year={2018},
  publisher={Springer}
}

@inproceedings{duggan2017predicting,
  title={Predicting host {CPU} utilization in cloud computing using recurrent neural networks},
  author={Duggan, Martin and Mason, Karl and Duggan, Jim and Howley, Enda and Barrett, Enda},
  booktitle={2017 12th International Conference for Internet Technology and Secured Transactions (ICITST)},
  pages={67--72},
  year={2017},
  organization={IEEE}
}

@article{blei2017variational,
  title={Variational inference: A review for statisticians},
  author={Blei, David M and Kucukelbir, Alp and McAuliffe, Jon D},
  journal={Journal of the American statistical Association},
  volume={112},
  number={518},
  pages={859--877},
  year={2017},
  publisher={Taylor \& Francis}
}

@book{hyndman2018forecasting,
  title={Forecasting: principles and practice},
  author={Hyndman, Rob J and Athanasopoulos, George},
  year={2018},
  publisher={OTexts}
}

@article{barati2015hybrid,
  title={A hybrid heuristic-based tuned support vector regression model for cloud load prediction},
  author={Barati, Masoud and Sharifian, Saeed},
  journal={The Journal of Supercomputing},
  volume={71},
  number={11},
  pages={4235--4259},
  year={2015},
  publisher={Springer}
}

@inproceedings{zhang2016workload,
  title={Workload prediction for cloud cluster using a recurrent neural network},
  author={Zhang, Weishan and Li, Bo and Zhao, Dehai and Gong, Faming and Lu, Qinghua},
  booktitle={2016 International Conference on Identification, Information and Knowledge in the Internet of Things (IIKI)},
  pages={104--109},
  year={2016},
  organization={IEEE}
}

@article{kumar2019efficient,
  title={An efficient machine learning approach for virtual machine resource demand prediction},
  author={Kumar, J and Singh, AK},
  journal={International Journal of Advanced Science and Technology},
  volume={123},
  pages={21--30},
  year={2019}
}

@inproceedings{kumar2019cloud,
  title={Cloud resource demand prediction using differential evolution based learning},
  author={Kumar, Jitendra and Singh, Ashutosh Kumar},
  booktitle={2019 7th International Conference on Smart Computing \& Communications (ICSCC)},
  pages={1--5},
  year={2019},
  organization={IEEE}
}

@inproceedings{wang2021predicting,
  title={Predicting {CPU} usage for proactive autoscaling},
  author={Wang, Thomas and Ferlin, Simone and Chiesa, Marco},
  booktitle={Proceedings of the 1st Workshop on Machine Learning and Systems},
  pages={31--38},
  year={2021}
}

@article{zhang2017resource,
  title={Resource requests prediction in the cloud computing environment with a deep belief network},
  author={Zhang, Weishan and Duan, Pengcheng and Yang, Laurence T and Xia, Feng and Li, Zhongwei and Lu, Qinghua and Gong, Wenjuan and Yang, Su},
  journal={Software: Practice and Experience},
  volume={47},
  number={3},
  pages={473--488},
  year={2017},
  publisher={Wiley Online Library}
}

@article{herbst2014self,
  title={Self-adaptive workload classification and forecasting for proactive resource provisioning},
  author={Herbst, Nikolas Roman and Huber, Nikolaus and Kounev, Samuel and Amrehn, Erich},
  journal={Concurrency and computation: practice and experience},
  volume={26},
  number={12},
  pages={2053--2078},
  year={2014},
  publisher={Wiley Online Library}
}

@article{zhou2020accurate,
  title={An Accurate Ensemble Forecasting Approach for Highly Dynamic Cloud Workload With VMD and R-Transformer},
  author={Zhou, Shaojing and Li, Jinguo and Zhang, Kai and Wen, Mi and Guan, Qijie},
  journal={IEEE Access},
  volume={8},
  pages={115992--116003},
  year={2020},
  publisher={IEEE}
}

@inproceedings{liu2016quantitative,
  title={Quantitative workload analysis and prediction using Google cluster traces},
  author={Liu, Bingwei and Lin, Yinan and Chen, Yu},
  booktitle={2016 IEEE Conference on Computer Communications Workshops (INFOCOM WKSHPS)},
  pages={935--940},
  year={2016},
  organization={IEEE}
}

@article{liu2020probabilistic,
  title={Probabilistic spatiotemporal wind speed forecasting based on a variational Bayesian deep learning model},
  author={Liu, Yongqi and Qin, Hui and Zhang, Zhendong and Pei, Shaoqian and Jiang, Zhiqiang and Feng, Zhongkai and Zhou, Jianzhong},
  journal={Applied Energy},
  volume={260},
  pages={114259},
  year={2020},
  publisher={Elsevier}
}

@article{khan2006bayesian,
  title={Bayesian neural network for rainfall-runoff modeling},
  author={Khan, Mohammad Sajjad and Coulibaly, Paulin},
  journal={Water Resources Research},
  volume={42},
  number={7},
  year={2006},
  publisher={Wiley Online Library}
}

@article{xie2007predicting,
  title={Predicting motor vehicle collisions using Bayesian neural network models: An empirical analysis},
  author={Xie, Yuanchang and Lord, Dominique and Zhang, Yunlong},
  journal={Accident Analysis \& Prevention},
  volume={39},
  number={5},
  pages={922--933},
  year={2007},
  publisher={Elsevier}
}

@article{lampinen2001bayesian,
  title={Bayesian approach for neural networks—review and case studies},
  author={Lampinen, Jouko and Vehtari, Aki},
  journal={Neural networks},
  volume={14},
  number={3},
  pages={257--274},
  year={2001},
  publisher={Elsevier}
}

@article{reiss2011google,
  title={Google cluster-usage traces: format+ schema},
  author={Reiss, Charles and Wilkes, John and Hellerstein, Joseph L},
  journal={Google Inc., White Paper},
  volume={1},
  year={2011}
}



@TechReport{clusterdata:Wilkes2020a,
  author = {John Wilkes},
  title = {{Google} cluster-usage traces v3},
  institution = {Google Inc.},
  year = 2020,
  month = Apr,
  type = {Technical Report},
  address = {Mountain View, CA, USA},
  note = {Posted at \url{https://github.com/google/cluster-data/blob/master/ClusterData2019.md}},
  abstract = {
	This document describes the semantics, data format, and
	schema of usage traces of a few Google compute cells.
	This document describes version 3 of the trace format.},
}

@article{jiang2020characterizing,
  title={Characterizing co-located workloads in alibaba cloud datacenters},
  author={Jiang, Congfeng and Qiu, Yitao and Shi, Weisong and Ge, Zhefeng and Wang, Jiwei and Chen, Shenglei and Cerin, Christophe and Ren, Zujie and Xu, Guoyao and Lin, Jiangbin},
  journal={IEEE Transactions on Cloud Computing},
  year={2020},
  publisher={IEEE}
}

@inproceedings{weng2022mlaas,
  title={{MLaaS} in the Wild: Workload Analysis and Scheduling in Large-Scale Heterogeneous {GPU} Clusters},
  author={Weng, Qizhen and Xiao, Wencong and Yu, Yinghao and Wang, Wei and Wang, Cheng and He, Jian and Li, Yong and Zhang, Liping and Lin, Wei and Ding, Yu},
  booktitle={19th USENIX Symposium on Networked Systems Design and Implementation (NSDI 22)},
  pages={945--960},
  year={2022}
}

@inproceedings{janardhanan2017cpu,
  title={{CPU} workload forecasting of machines in data centers using {LSTM} recurrent neural networks and {ARIMA} models},
  author={Janardhanan, Deepak and Barrett, Enda},
  booktitle={2017 12th International Conference for Internet Technology and Secured Transactions (ICITST)},
  pages={55--60},
  year={2017},
}

@article{mireslami2019dynamic,
  title={Dynamic cloud resource allocation considering demand uncertainty},
  author={Mireslami, Seyedehmehrnaz and Rakai, Logan and Wang, Mea and Far, Behrouz H},
  journal={IEEE Transactions on Cloud Computing},
  volume={9},
  number={3},
  pages={981-994},
  year={2019},
  publisher={IEEE}
}

@inbook{han2011data,
  title={Data mining: concepts and techniques},
  author={Han, Jiawei and Pei, Jian and Kamber, Micheline},
  year={2011},
  publisher={Elsevier},
  pages = {111-118}
}

@article{bollerslev1986generalized,
  title={Generalized autoregressive conditional heteroskedasticity},
  author={Bollerslev, Tim},
  journal={Journal of econometrics},
  volume={31},
  number={3},
  pages={307--327},
  year={1986},
  publisher={Elsevier}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{fawaz2019deep,
  title={Deep learning for time series classification: a review},
  author={Fawaz, Hassan Ismail and Forestier, Germain and Weber, Jonathan and Idoumghar, Lhassane and Muller, Pierre-Alain},
  journal={Data mining and knowledge discovery},
  volume={33},
  number={4},
  pages={917--963},
  year={2019},
  publisher={Springer}
}

@inproceedings{blundell2015weight,
  title={Weight uncertainty in neural network},
  author={Blundell, Charles and Cornebise, Julien and Kavukcuoglu, Koray and Wierstra, Daan},
  booktitle={International Conference on Machine Learning},
  pages={1613--1622},
  year={2015},
  organization={PMLR}
}

@article{joyce2011kullback,
  title={Kullback-Leibler Divergence.},
  author={Joyce, James M},
  journal={International encyclopedia of statistical science},
  volume={720},
  pages={722},
  year={2011}
}

@article{zeng2018relevance,
  title={The relevance of Bayesian layer positioning to model uncertainty in deep Bayesian active learning},
  author={Zeng, Jiaming and Lesnikowski, Adam and Alvarez, Jose M},
  journal={arXiv preprint arXiv:1811.12535},
  year={2018}
}

@article{brosse2020last,
  title={On last-layer algorithms for classification: Decoupling representation from uncertainty estimation},
  author={Brosse, Nicolas and Riquelme, Carlos and Martin, Alice and Gelly, Sylvain and Moulines, {\'E}ric},
  journal={arXiv preprint arXiv:2001.08049},
  year={2020}
}

@article{hullermeier2021aleatoric,
  title={Aleatoric and epistemic uncertainty in machine learning: An introduction to concepts and methods},
  author={H{\"u}llermeier, Eyke and Waegeman, Willem},
  journal={Machine Learning},
  volume={110},
  number={3},
  pages={457--506},
  year={2021},
  publisher={Springer}
}

@inproceedings{mao2010cloud,
  title={Cloud auto-scaling with deadline and budget constraints},
  author={Mao, Ming and Li, Jie and Humphrey, Marty},
  booktitle={2010 11th IEEE/ACM International Conference on Grid Computing},
  pages={41--48},
  year={2010},
  organization={IEEE}
}

@article{koutsandreas2021selection,
  title={On the selection of forecasting accuracy measures},
  author={Koutsandreas, Diamantis and Spiliotis, Evangelos and Petropoulos, Fotios and Assimakopoulos, Vassilios},
  journal={Journal of the Operational Research Society},
  pages={1--18},
  year={2021},
  publisher={Taylor \& Francis}
}

@book{shmueli2017data,
  title={Data mining for business analytics: concepts, techniques, and applications in R},
  author={Shmueli, Galit and Bruce, Peter C and Yahav, Inbal and Patel, Nitin R and Lichtendahl Jr, Kenneth C},
  year={2017},
  publisher={John Wiley \& Sons}
}

@inbook{sarkar2018hands,
  title={Hands-On Transfer Learning with Python: Implement advanced deep learning and neural network models using TensorFlow and Keras},
  author={Sarkar, Dipanjan and Bali, Raghav and Ghosh, Tamoghna},
  year={2018},
  pages={166--168},
  publisher={Packt Publishing Ltd}
}

@article{ardagna2014quality,
  title={Quality-of-service in cloud computing: modeling techniques and their applications},
  author={Ardagna, Danilo and Casale, Giuliano and Ciavotta, Michele and P{\'e}rez, Juan F and Wang, Weikun},
  journal={Journal of Internet Services and Applications},
  volume={5},
  number={1},
  pages={1--17},
  year={2014},
  publisher={SpringerOpen}
}

@article{minarolli2017tackling,
  title={Tackling uncertainty in long-term predictions for host overload and underload detection in cloud computing},
  author={Minarolli, Dorian and Mazrekaj, Artan and Freisleben, Bernd},
  journal={Journal of Cloud Computing},
  volume={6},
  number={1},
  pages={1--18},
  year={2017},
  publisher={Springer}
}

@inproceedings{minarolli2014cross,
  title={Cross-correlation prediction of resource demand for virtual machine resource allocation in clouds},
  author={Minarolli, Dorian and Freisleben, Bernd},
  booktitle={2014 Sixth International Conference on Computational Intelligence, Communication Systems and Networks},
  pages={119--124},
  year={2014},
  organization={IEEE}
}

@article{neyshabur2017exploring,
  title={Exploring generalization in deep learning},
  author={Neyshabur, Behnam and Bhojanapalli, Srinadh and McAllester, David and Srebro, Nati},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{alashhab2021impact,
  title={Impact of coronavirus pandemic crisis on technologies and cloud computing applications},
  author={Alashhab, Ziyad R and Anbar, Mohammed and Singh, Manmeet Mahinderjit and Leau, Yu-Beng and Al-Sai, Zaher Ali and Alhayja’a, Sami Abu},
  journal={Journal of Electronic Science and Technology},
  volume={19},
  number={1},
  pages={100059},
  year={2021},
  publisher={Elsevier}
}
